Deep Double Descent: Where Bigger Models and More Data Hurt

We show that a variety of modern deep learning tasks exhibit a "double-descent" phenomenon where, as we increase model size, performance first gets worse and then gets better. Moreover, we show that double descent occurs not just as a function of model size, but also as a function of the number of training epochs. We unify the above phenomena by defining a new complexity measure we call the effective model complexity and conjecture a generalized double descent with respect to this measure. Furthermore, our notion of model complexity allows us to identify certain regimes where increasing (even quadrupling) the number of train samples actually hurts test performance.

==> general_dd.tex <==
\section{Generalized Double Descent}
\label{sec:general}

Here we present a generic (though informal) way of unifying the three types of
double-descent phenomenon we observe. In particular, we introduce a notion of ``Effective Model Complexity'' along which double-descent occurs.

\pnote{Todo, rewrite this.}

\begin{definition}[Learning Algorithm]
A \emph{learning algorithm $\cA$}
$$\cA: (\cX \x \cY)^* \to M$$
is a function mapping $n$ samples $\{(x_i, y_i)\}$
to a \emph{Model} $M: \cX \to \cY$.
\end{definition}
We will consider learning-algorithms which take as input
$n$ i.i.d. samples $(x_i, y_i) \sim \cD$ from a distribution $\cD$,
and output a model $M$ (for example, by training a neural-network via SGD on the samples).


\begin{definition}[Model Complexity]
For a learning-algorithm $\cA$, distribution $\cD$, loss function $\cL$, and $0 \leq \eps \ll 1$,
define the 
\emph{ModelComplexity}$_{\cD, \cL, \eps}(\cA)$
as the maximum number of samples from $\cD$ for which $\cA$ outputs a model with small train loss.
Formally,
$$
\mathrm{ModelComplexity}_{\cD, \cL, \eps}(\cA)
:=
\argmax_n  \Pr_{\substack{
\{(x_i, y_i)\} \sim \cD^n\\
M \gets \cA(\{(x_i, y_i)\})
}}\left[ \frac{1}{n} \sum_i \cL( M(x_i), y_i )  \leq \eps \right] \geq 1-o(1)
$$
\end{definition}

Throughout, we consider learning-algorithms which output models by 
training a neural network, optimizing the train loss via SGD or variants.
In this case, let $\cA_{NN}[\text{Model-Size, Train-Steps}]$ be the learning algorithm
which trains a neural-network of a given size and architecture for the given number of train steps.

For $n$ training samples,
we consider a learning-algorithm $\cA$ to be ``overparmeterized'' if
$$
\mathrm{ModelComplexity}_{\cD, \cL, \eps}(\cA)
\gg n
$$
and ``underparameterized'' if
$\mathrm{ModelComplexity}_{\cD, \cL, \eps}(\cA) \ll n$,
and ``critically parameterized'' if
$\mathrm{ModelComplexity}_{\cD, \cL, \eps}(\cA) \approx n$.


We can now state our main thesis in terms of the above.
\begin{claim}[Phase Transision, Informal]
Neural-network learning algorithms $\cA_{NN}$ undergo
a \emph{phase transition} in their test performance 
in the ``critically parameterized'' regime, when
the \emph{ModelComplexity} is equal to the size of the train set.
That is, when
$$
\mathrm{ModelComplexity}_{\cD, \cL, \eps}(\cA_{NN})
= n
$$
where $n$ is the number of training examples.
\end{claim}




==> more_discussion.tex <==
\section{On The Mechanisms and Characterizations of Double Descent}
\label{sec:morediscuss}

\paragraph{On Effective Model Complexity.}
We stress that Effective Model Complexity is \emph{not} a single-letter characterization
of test error.
For example, two training procedures with the same EMC can output models with
very different test errors (e.g. consider a CNN and a fully-connected net, which both are capable of interpolating the same number of samples from a natural image distribution.
Here, we would expect the CNN to have much lower test error than the fully-connected net.
Our generalized double desccent hypothesis applies as we vary EMC in a ``smooth'' way--- say, by only
changing the model by a small amount--- and does not apply if we say, jump discontinuously from a CNN to a fully-connected net.
